A measurement of the group velocity of scintillation light in liquid argon

The propagation velocity of scintillation light in liquid argon $v_{g}$ at $\lambda \sim 128$~nm wavelength, has been measured for the first time in a dedicated experimental setup at CERN.\\ The obtained result $\frac{1}{v_{g}} = 7.46 \pm 0.08$~ns/m , is then used to derive the value of the refractive index (n) and the Rayleigh scattering length ($\mathcal{L}$) for liquid argon in the VUV region. For $\lambda = 128$~nm we found $n= 1.358 \pm 0.003$ and $\mathcal{L}= 99.1 \pm 2.3$~cm. The measured values are of interest for a variety of experiments searching for rare events like neutrino and dark matter interactions. The derived quantities also represent key information for theoretical models describing the propagation of scintillation light in liquid argon.

==> reference.tex <==
\begin{thebibliography}{99}
\footnotesize
%\bibitem{1a}
%J. Beringer {\it et al.}, (Particle Data Group), The Review of Particle Physics,
%Phys. Rev. D 86 (2012).

\bibitem{SBN}
R Acciarri {\it et al.}, A Proposal for a Three Detector Short-Baseline Neutrino Oscillation Program in the Fermilab Booster Neutrino Beam, arXiv:1503.01520 [physics.ins-det].

\bibitem{DUNE}
R Acciarri {\it et al.}, DUNE/LBNF CDR Volume 1: The LBNF and DUNE Projects, arXiv:1601.05471 [physics.ins-det].

\bibitem{DarkSide}
P.D.Meyersfor the DarkSide Collaboration, DarkSide-50: A WIMP Search with a Two-phase Argon TPC, Physics Procedia 61, 124 - 129 (2015).

\bibitem{light_production_exp}
T Heindl {\it et al.}, The scintillation of liquid argon, EPL 91, 62002 (2010).

\bibitem{LArLight_plot}
E. Morikawa, R. Reininger  {\it et al.}, Argon, krypton, and xenon excimer luminescence: From the dilute gas to the
condensed phase, The Journal of Chemical Physics 91, 1469 (1989).

\bibitem{LArFilippo}
O. Cheshnovsky et al., Emission Spectra of Deep Impurity States in Solid and Liquid Rare Gas Alloys, J. Chem. Phys., 57 (1972) 4628.


\bibitem{QE}
ICARUS Collaboration (M. Babicz \it{et al.}), \textit{Test and characterization of 400 Hamamatsu R5912-MOD photomultiplier tubes for the ICARUS T600 detector}, JINST 13 P10030 (2018).

\bibitem{GL}
G.L. Raselli \it{et al.}, \textit{Test and characterization of 20 pre-series hamamatsu R5916-MOD photomultiplier tubes for the ICARUS T600 detector},journal={2016 IEEE Nuclear Science Symposium, Medical Imaging Conference and Room-Temperature Semiconductor Detector Workshop (NSS/MIC/RTSD),}% 10.1109/NSSMIC.2016.8069768}.

\bibitem{light_production_exp2}
T Heindl {\it et al.}, \textit{Table-top setup for investigating the scintillation properties of liquid argon}, JINST 6 P02011 (2011).

\bibitem{light_production_exp3}
M. Hofmann {\it et al.}, \textit{Ion-beam excitation of liquid argon}, EPJ-C 73, 2618 (2013).

\bibitem{Rayleigh_th}
G. Seidel, R. Lanou, W. Yao, \textit{Rayleigh scattering in rare-gas liquids}, NIM A 489, 189 - 194 (2002).

\bibitem{refIndex} A. Bideau-Mehu, Y. Guern, {\it et al.}, Measurement of refractive indices of neon, argon, krypton and xenon in the 253.7–140.4 nm wavelength range. Dispersion relations and estimated oscillator strengths of the resonance lines, J. Quant. Spectrosc. Radiat. Transfer  25 395 (1981).

\bibitem{Hitachi} A. Hitachi {\it et al.}, New approach to the calculation of the refractive index of liquid and solid xenon, J. Chem. Phys. 123, 234508 (2005).

\bibitem{Rayleigh_th2}
E. Grace {\it et al.}, Index of refraction, Rayleigh scattering length, and Sellmeier coefficients in solid and liquid argon and xenon, \href{ 10.1016/j.nima.2017.06.031}{NIM A867 (2017) 204-208}.

\bibitem{Rayleigh_exp}
N. Ishida {\it et al.}, Attenuation length measurements of scintillation light in liquid rare gases and their mixtures using an improved reflection suppresser, NIM A 384, 380 – 386 (1997).

\bibitem{ArDM}
ArDM Collaboration (J. Calvo et al.), \textit{Measurement of the attenuation length of argon scintillation light in the ArDM LAr TPC, }\href{10.1016/j.astropartphys.2017.11.009}{Astropart.Phys. 97 (2018) 186-196.}

\bibitem{ANeumeier}
A. Neumeier et al., \textit{Attenuation of vacuum ultraviolet light in pure and xenon-doped liquid argon - an approach to an assignment of the near-infrared emission from the mixture, }\href{http://iopscience.iop.org/article/10.1209/0295-5075/111/12001/pdf}{2015 EPL 111 12001.}

\bibitem{energy_levels_Ar2}
J. H. Yates {\it et al.}, Ab initio potential energy curves for the low-lying electronic states of the argon excimer, The Journal of Chemical Physics 79, 6145 (1983).

\bibitem{Maurathesis}
M. Spanu, Study on the TPB as wavelength shifter for the ICARUS T600 light detection system in the Fermilab SBN project, Universita degli studi di Pavia, Ph.D XXX ciclo (2018). 

\bibitem{ICARUSPMTs}
M.Babicz, V. Bellini,  {\it et al.},  \textit{Timing properties of Hamamatsu R5912-MOD photomultiplier tube for the ICARUS T600 light detection system}, NIM-A, Volume 912, (2018) 231-234.

\bibitem{PMTsaturation}
M.Babicz, V. Bellini,  {\it et al.},  \textit{Linearity and saturation properties of Hamamatsu R5912-MOD photomultiplier tube for the ICARUS T600 light detection system}, NIM-A, A 936 (2019) 554–555.

\bibitem{GL2}
M.Bonesini {\it et al.}, \textit{An innovative technique for TPB deposition on convex window photomultiplier tubes}, JINST 13, P12020 (2018).

\bibitem{Doke}
T. Doke {\it et al.}, Absolute Scintillation Yields in Liquid Argon and Xenon for Various Particles, Jpn. J. Appl. Phys. 41, 1538 (2002).

\bibitem{SinnockSmith}
A. C. Sinnock, B. L. Smith, \textit{Refractive indices of the condensed rare gases, argon, krypton and xenon, } \href{https://doi.org/10.1088/0022-3719/13/12/018}{1980 J. Phys. C: Solid State Phys. 13 2375}.


\bibitem{BideuMehu}
A.Bideau-MehuY.GuernR.AbjeanA.Johannin-Gilles, \textit{Measurement of refractive indices of neon, argon, krypton and xenon in the 253.7 - 140.4 nm wavelength range. Dispersion relations and estimated oscillator strengths of the resonance lines, }\href{https://doi.org/10.1016/0022-4073(81)90057-1}{Journal of Quantitative Spectroscopy and Radiative Transfer 25 (1981) 395 - 402}.


\bibitem{LArBook}
https://encyclopedia.airliquide.com/argon

\bibitem{Mavrokoridis}
Mavrokoridis, K. \it{et al.} Argon Purification Studies and a Novel Liquid Argon Re-circulation System, JINST 6, (2011) P08003 arXiv:1106.5226 [physics.ins-det].

\bibitem{FLUKA1}
A. Ferrari, P.R. Sala, A. Fasso`, and J. Ranft,
FLUKA: a multi-particle transport code,
CERN 2005-10 (2005), INFN/TC\_05/11, SLAC-R-773 .

\bibitem{FLUKA2}
G. Battistoni et al. ,Overview of the FLUKA code,
Annals of Nuclear Energy 82, 10-18  (2015).

\bibitem{epl91-62002-2010}
 T. Heindl \it{et al.} The scintillation of liquid argon, European Physics Letter 91 62002, 2010.

\bibitem{N2contaminationLAr}
R Acciarri {\it et al.}, Effects of Nitrogen contamination in liquid Argon, JINST  5 P06003 (2010). 

\bibitem{LarLightcollection}
V. Boccone, C. Amsler {\it et al.},  Light Readout for a 1 ton Liquid Argon Dark Matter Detector, http://cds.cern.ch/record/1276774.
  
\bibitem{FitScintForm}
  E.H.Bellamy et al., Absolute calibration and monitoring of a spectrometric channel using a photomultiplier, \href{https://doi.org/10.1016/0168-9002(94)90183-X}{Nucl. Instrum. Meth., in Phys. Res. A 339(1994) 468-476.}
  
  \bibitem{Landau}
 L.D. Landau and E.M. Lifshitz. volume 8. Pergamon Press, 1960.

\bibitem{Bornbook}
M. Born, E. Wolf, Principles of Optics, 7th Edition, Cambridge University Press, 1999.


\end{thebibliography}
